To Regularize or Not To Regularize? The Bias Variance Trade-off in Regularized AEs

Regularized Auto-Encoders (RAEs) form a rich class of neural generative models. They effectively model the joint-distribution between the data and the latent space using an Encoder-Decoder combination, with regularization imposed in terms of a prior over the latent space. Despite their advantages, such as stability in training, the performance of AE based models has not reached the superior standards as that of the other generative models such as Generative Adversarial Networks (GANs). Motivated by this, we examine the effect of the latent prior on the generation quality of deterministic AE models in this paper. Specifically, we consider the class of RAEs with deterministic Encoder-Decoder pairs, Wasserstein Auto-Encoders (WAE), and show that having a fixed prior distribution, \textit{a priori}, oblivious to the dimensionality of the `true' latent space, will lead to the infeasibility of the optimization problem considered. Further, we show that, in the finite data regime, despite knowing the correct latent dimensionality, there exists a bias-variance trade-off with any arbitrary prior imposition. As a remedy to both the issues mentioned above, we introduce an additional state space in the form of flexibly learnable latent priors, in the optimization objective of the WAEs. We implicitly learn the distribution of the latent prior jointly with the AE training, which not only makes the learning objective feasible but also facilitates operation on different points of the bias-variance curve. We show the efficacy of our model, called FlexAE, through several experiments on multiple datasets, and demonstrate that it is the new state-of-the-art for the AE based generative models.

==> abstract.tex <==
Auto-Encoder based models form a rich class of techniques for generating samples from an underlying data distribution. They model the joint-likelihood using an encoder-decoder combination, with regularization imposed in terms of a prior over the latent space. While the original set of models, i.e., VAE~\cite{},AAE~\cite{}, made the assumption of a Gaussian prior over the latent, a number of methods have been proposed which argue for the insufficiency of the Gaussian prior for the generative task, and have come up with more sophisticated priors to improve generation quality. Though this has pushed the state-of-the-art, we argue in this paper, existing literature lacks a systematic treatment to what an ideal prior should be for a given AE based model. We pose this as a problem of trade-off between bias and variance, and show that no single prior can be optimal (in terms of achieving the max data likelihood) when using a Gaussian encoder/decoder, for all data distributions. As a remedy, we propose a generalized ELBO objective, which parameterizes over the latent prior, in addition to the encoder and decoder parameters. We jointly learn this prior using a finite capacity GAN, coupled with the original encoder-decoder combination. All previously proposed (parametric?) priors come out as a special case of our GAN based framework, by the way of universal approximation theorem. In the limit of increasing capacity, our GAN is able to learn arbitrary priors, achieving the bound on maximum data likelihood, though it comes at the cost of over-fitting when learning with finite samples. Controlling the capacity of our GAN gives us a handle to trade-off between bias and variance. Our experiments on a number of generation tasks, show that our prior learning framework is the new state-of-the-art for AE based models, and achieves FID scores comparable to pure GAN based generative models, while still retaining the nice properties of AE architectures. 

%are a special case of our GAN based architecture.  

